Reinforcing Action Policies by Prophesying

Vision-Language-Action (VLA) policies excel in aligning language, perception, and robot control. However, most VLAs are trained purely by imitation, which overfits to demonstrations, and is brittle under distribution shift. Reinforcement learning (RL) directly optimizes task reward and thus addresses this misalignment, but real-robot interaction is expensive and conventional simulators are hard to engineer and transfer. We address both data efficiency and optimization stability in VLA post-training via a learned world model and an RL procedure tailored to flow-based action heads. Specifically, we first introduce Prophet, a unified action-to-video robot world model pretrained on large-scale, heterogeneous robot data to learn reusable action-outcome dynamics and then few-shot adapted to new robots, objects, and environments, yielding a rollout-ready simulator. Upon Prophet, we reinforce action policies with our proposed FlowScale, which couples Flow-GRPO with intrinsic stepwise reweighting to stabilize gradients. Together, our solution provides a practical, data- and compute-efficient path to VLA post-training. Experiments show 5-17% success gains on public benchmarks and 24-30% on real robots across diverse VLA backbones.

==> tables/rm_reward_control.tex <==
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{0.95}
\caption{\textbf{Reward control on LIBERO Spatial simulator RL.}
All rows use VLA-Adapter in the simulator-only setting of Tab.~\ref{tab:rl_ablation}.}
\scalebox{0.9}{
\begin{tabular}{lc}
\toprule
\textbf{Setting} & Success$\uparrow$ \\
\midrule
VLA-Adapter SFT & $82.7 \pm 0.9$ \\
Simulator RL w/ GT reward & $94.6 \pm 1.2$ \\
Simulator RL w/ 72B RM & $90.4 \pm 0.6$ \\
\bottomrule
\end{tabular}
}
\label{tab:sim_rm_control}
\end{table}

